Learning to Detect Few-Shot-Few-Clue Misinformation

The quality of digital information on the web has been disquieting due to the lack of careful manual review. Consequently, a large volume of false textual information has been disseminating for a long time since the prevalence of social media. The potential negative influence of misinformation on the public is a growing concern. Therefore, it is strongly motivated to detect online misinformation as early as possible. Few-shot-few-clue learning applies in this misinformation detection task when the number of annotated statements is quite few (called few shots) and the corresponding evidence is also quite limited in each shot (called few clues). Within the few-shot-few-clue framework, we propose a Bayesian meta-learning algorithm to extract the shared patterns among different topics (i.e.different tasks) of misinformation. Moreover, we derive a scalable method, i.e., amortized variational inference, to optimize the Bayesian meta-learning algorithm. Empirical results on three benchmark datasets demonstrate the superiority of our algorithm. This work focuses more on optimizing parameters than designing detection models, and will generate fresh insights into data-efficient detection of online misinformation at early stages.

==> 5-method-0.tex <==

\section{Methodology}
\label{{sec:method}}
After formulating the task of early misinformation detection as a few-shot-few-clue problem, we propose a Bayesian meta-learning based framework to solve this problem.
Under this framework, neural networks are implemented to encode statements to be verified and their corresponding clues. Figure~\ref{fig:neural_encoder} describes how neural encoders produce representations and predictions. Note that neural network weights are local parameters $\boldsymbol{\phi}$, and in the Bayesian meta-learning framework, are random variables. 
Therefore, these neural encoders are Bayesian neural networks in nature and are able to capture uncertainty existing in datasets. 

\label{sec:method}
\begin{figure*}[th]
\center
\includegraphics[width=0.9\textwidth]{figures/framework.pdf}
\caption{Neural modules to produce representations and predictions, consisting of two parts, the statement encoder (\S~\ref{sec:encoding_statement}) and the clue encoder (\S~\ref{sec:encoding_clues}), the concatenation of which determines the statement veracity. 
Blocks of the same color denote the same computational modules.
% Grey nodes are observed variables while blank nodes are latent variables (similarly with Figure~\ref{fig:metaGraphicalRepresentation}).
}
\label{fig:neural_encoder}
\end{figure*}

\subsection{Encoding Statement}
\label{sec:encoding_statement}
An input datum consists of two elements: a statement to be verified and its clues. 
The statement is a sequence of words, the linguistic features of which are a strong indicator of its veracity. We aim to capture such features by neural networks. 
% For simplicity, we omit the task $\tau$ in following derivations.

For a task $\tau$ with $M^\tau$ data, the statement of the $m$-th ($1\leq m\leq M^\tau$) datum can be denoted as $\boldsymbol{s}_m^\tau=[\boldsymbol{w}_1, \dots, \boldsymbol{w}_l]$, where $\boldsymbol{w}_l \in \mathbb{R}^d$ is a $d$-dimensional pre-trained word embedding.
Then, the embedding sequence is input to a commonly used Bidirectional Long Short Term Memory (BiLSTM) neural network~\cite{graves2005bidirectional}, which extracts linguistic features both from previous time steps and future time steps via forward and backward states. The output of the BiLSTM is a concatenation of these two states summarizing past and future information:
%Its output are two hidden states that capture the past and the future information. We concatenate the last hidden states from two directions to form the output of the BiLSTM: 
\begin{align}
\vec{\boldsymbol{h}}_s^{m,\tau} &= \overrightarrow{\mathrm{LSTM}}(\boldsymbol{s}_m^\tau; \boldsymbol{\phi}^\tau),\\
\cev{\boldsymbol{h}}_s^{m,\tau} &= \overleftarrow{\mathrm{LSTM}}(\boldsymbol{s}_m^\tau; \boldsymbol{\phi}^\tau),\\
\boldsymbol{h}_s^{m,\tau} & =[\vec{\boldsymbol{h}}_s^{m,\tau},\cev{\boldsymbol{h}}_s^{m,\tau}],
\end{align}
% \begin{equation}
% \boldsymbol{h}_s  ={\mathrm{BiLSTM}}(\boldsymbol{s}),
% \end{equation}
where $\vec{\boldsymbol{h}}_s^{m,\tau}$ and $\cev{\boldsymbol{h}}_s^{m,\tau}$ represent the last states of forward $\overrightarrow{\mathrm{LSTM}}$ and backward $\overleftarrow{\mathrm{LSTM}}$ directions respectively. $\boldsymbol{h}_s^{m,\tau}$ denotes the dense representation of concatenated hidden states.


\subsection{Encoding Clues}
\label{sec:encoding_clues}
%\vspace{1em}
In order to verify whether a statement is true or false, a mostly adopted approach is to make use of auxiliary evidences or clues~\cite{popat2018declare,zhang2019reply}. Similar to the statement encoder, the clue encoder is also implemented as neural networks. However, there are two differences: (1) there are usually more than one clues with each as a sequence of words, and (2) clues from credible sources can be more contributive. Accordingly, we incorporate source features into clue representations.

Given a set of clues $\mathcal{C}_m^\tau=\left\{\boldsymbol{c}_{m,1}^\tau,\ldots,\boldsymbol{c}_{m,n}^\tau,\ldots, \boldsymbol{c}_{m,N}^\tau\right\}$, 
% 
where $\boldsymbol{c}_{m,n}^\tau$ denotes a sequence of words $\boldsymbol{c}_{m,n}^\tau =[\boldsymbol{w}_1,\dots, \boldsymbol{w}_k]$. 
To project the statement and clues into the same semantic space, we use the same pre-trained word embeddings for both statements and clues. 
Hence, $\boldsymbol{w}_k \in \mathbb{R}^d$ is a $d$-dimensional vector such as the word embedding vector used to encoding the statement.
For the sake of semantic coherence, we also employ the same BiLSTM to encode both the statement and its clues. 
Take the clue $\boldsymbol{c}_{m,n}^\tau \in \mathcal{C}_m^\tau$ for example, the concatenation of hidden states from forward and backward directions is denoted as: 
\begin{align}
\vec{\boldsymbol{h}}_{c_n}^{m,\tau} &=  \overrightarrow{\mathrm{LSTM}}(\boldsymbol{c}_{m,n}^\tau; \boldsymbol{\phi}^\tau),\\
\cev{\boldsymbol{h}}_{c_n}^{m,\tau} &=  \overleftarrow{\mathrm{LSTM}}(\boldsymbol{c}_{m,n}^\tau; \boldsymbol{\phi}^\tau),\\
\boldsymbol{h}_{c_n}^{m,\tau} &= [\vec{\boldsymbol{h}}_{c_n}^{m,\tau},\cev{\boldsymbol{h}}_{c_n}^{m,\tau}],
\end{align}
% \begin{equation}
% \boldsymbol{h}_{c_n} = \mathrm{BiLSTM}(\boldsymbol{c}_{m,n}^\tau),
% \end{equation}
where $\boldsymbol{h}_{c_n}^{m,\tau}$ is the summary of the clue $\boldsymbol{c}_{m,n}^\tau$.

As there are usually more than one clue for each statement, we need to integrate them. One possible way is to obtain a dense representation that summarizes all clues along the time line, emphasizing on the more recent clues. However, this way ignores the influence of source credibility. On contrast, we assign each unique source to an embedding and concatenate this source embedding to the clue embedding,  
\begin{equation}
\boldsymbol{h}_{a_n}^{m,\tau} = \mathrm{Emb}(\boldsymbol{a}_{m,n}^\tau; \boldsymbol{\phi}^\tau),
\end{equation}
where $\boldsymbol{a}_{m,n}^\tau$ is the one-hot representation for the source of the $n$-th clue, $\mathrm{Emb}$ is an embedding module and $\boldsymbol{h}_{a_n}^{m,\tau}$ is the dense source embedding.

% clues on social media platforms are listed along the time line , where the earliest clue appears at the top of the list. 
% Truth about an event can be gradually manifest as more evidence emerges, thus we assume that the latest clues tend to be more reliable and more important than the earlier clues. Based on this assumption, we design a two-layer recurrent neural network to encode clues: the first-layer applies a BiLSTM to summarize the semantic information of each clue and the second-layer applies a LSTM to capture the temporal semantic variation of the clues.



In order to capture the semantic information of all clues, we sequentially input the concatenated hidden states of each clue into a LSTM.
We use the LSTM rather than a BiLSTM because the former gives high weights to recent input, which matches our assumption on the relative importance of the latest clue. 
Specifically, the LSTM takes the hidden states of each clue as input in a sequential way:
% %
\begin{equation}
\label{eqn:h_d}
\boldsymbol{h}_{\mathcal{C}}^{m,\tau} = {\mathrm{LSTM}}(\boldsymbol{h}_{c,a}^N; \boldsymbol{\phi}^\tau),
\end{equation}
% %
where $\boldsymbol{h}_{c,a}^N=\{ 
[\boldsymbol{h}_{c_1}^{m,\tau},\boldsymbol{h}_{a_1}^{m,\tau}], \dots, [\boldsymbol{h}_{c_n}^{m,\tau},\boldsymbol{h}_{a_n}^{m,\tau}], \dots, [\boldsymbol{h}_{c_N}^{m,\tau},\boldsymbol{h}_{a_N}^{m,\tau}]\}$.

The hidden state $\boldsymbol{h}_{\mathcal{C}}^{m,\tau}$ contains the linguistic information of each clue, and is then used together with $\boldsymbol{h}_s^{m,\tau}$ to predict statement veracity. 



\subsection{Veracity Modeling}

In \S~\ref{sec:encoding_statement}, we obtain a dense representation $\boldsymbol{h}_s^{m,\tau}$ containing linguistic features of the statement. In this section we include clues to predict veracity.
%We show contribution of clues in the \S~\ref{sec:results}.

Veracity is predicted by combining the statement and clue information via a MLP. The strong non-linearity of MLPs make them suitable to find complex relationships between the statement and its clues.
Specifically, 
the MLP input is the statement representation $\boldsymbol{h}_s^{m,\tau}$ concatenated to the hidden state of clues $\boldsymbol{h}_{\mathcal{C}}^{m,\tau}$:
\begin{equation}
    y_m^\tau =\mathrm{MLP}(\boldsymbol{h}_s^{m,\tau},\boldsymbol{h}_{\mathcal{C}}^{m,\tau}; \boldsymbol{\phi}^\tau).
\end{equation}
This is the final prediction of our Bayesian meta-learning model for misinformation detection.

